Deimos: A Grammar of Dynamic Embodied Immersive Visualisation Morphs and Transitions

We present Deimos, a grammar for specifying dynamic embodied immersive visualisation morphs and transitions. A morph is a collection of animated transitions that are dynamically applied to immersive visualisations at runtime and is conceptually modelled as a state machine. It is comprised of state, transition, and signal specifications. States in a morph are used to generate animation keyframes, with transitions connecting two states together. A transition is controlled by signals, which are composable data streams that can be used to enable embodied interaction techniques. Morphs allow immersive representations of data to transform and change shape through user interaction, facilitating the embodied cognition process. We demonstrate the expressivity of Deimos in an example gallery and evaluate its usability in an expert user study of six immersive analytics researchers. Participants found the grammar to be powerful and expressive, and showed interest in drawing upon Deimos' concepts and ideas in their own research.

==> Letter_to_Reviewers_1.tex <==
Dear reviewers,

We would like to thank all of you for your kind and helpful feedback. We have opted to make significant changes to the manuscript to accommodate as many suggestions as possible. We list the following changes in the order which they appear in the manuscript. We have also provided a marked up version of the manuscript which highlights all of the changes made.

Most of Section 1 (Introduction) has been rewritten to omit the concept of embodied cognition (R1). We have also rewritten it in an attempt to further emphasise the novelty, significance, and importance of our work (2AC, R2). We do so by explaining the connection that (embodied) interaction has with animation through the notion of gestural congruency (R1). This connection strengthens the motivation as it is now twofold: arguing from the two research directions simultaneously (embodied interaction and animation). We also highlight the fact that no Immersive Analytics toolkit has yet provided means to rapidly prototype embodied interactions, despite the concept being intrinsic to Immersive Analytics. We also added several missing references relating to animation for visualisation literacy (R2).

While not directly requested by any reviewer, we rewrote almost the entirety of the Section 2 (Related Work) in order to better position our work to the literature. We also added a new subsection specifically on embodied interaction and metaphors (R1) to better explain and justify their use.

In Section 3 (Design Goals), we rephrased DG2 to be less about the grammar directly leveraging embodied interaction, but moreso supporting its use if desired by the morph designer. We also added further references here to strengthen the argument for embodied interaction and why it is important (R1). We also discussed how embodied interaction principles could be used in the context of Deimos: less as guidelines for how the grammar was designed and more as guidelines for the morph designer themselves (R1). Through this, Deimos becomes more of a testbed that can accommodate a range of designs, which also feeds into DG3.

We provided an explanation of how the Deimos grammar was created to ease the transition between Sections 3 (Design Goals) and 4 (Grammar) (R1).

The 2AC asked us to emphasise the difference between 2D and immersive visualisation. They also asked to highlight how the grammar handles these challenges. Both were meant to be served by Sections 3 and 4, but in hindsight were likely not explicit enough. As a result, Section 3 was reworded slightly to state that they are based on the differences and challenges stemming from the shift to immersive. We also decided to modify Section 4 to make clear the components which directly address the design goals and how. We also added a new Section 4.4 to reiterate these points, and forward references Section 6 (Example Gallery) that demonstrates clearly how the design goals were met.

R2 asked for clarification on how keyframes are created. This process was originally described in Section 4.1.2 (Keyframe Creation Process). Unfortunately as R2's comment was rather vague, we weren't sure how exactly to address it. We apologise in advance if this is a major issue. To clarify, our work generates keyframes using a set of heuristics. Gemini in comparison does so using a more complex recommendation system.

We added several sentences to explain what DXR is in Section 5.1 (Data Visualisations) (R1, R2). As we did not want to get into specifics about how DXR was implemented, we mainly described its original capabilities as a visualisation toolkit.

We tweaked several sentences in Section 6.2 (Embodied vs Non-embodied Example Gallery) to tie in some of the additions we made earlier in response to R1.

We added the types of questions we asked our participants in the semi-structured interview in Section 7.1 (Study Design) (R1).

We added two new topics to Section 8 (Discussion). One is based on R2's suggestion on data-driven vs interaction-driven animated transition grammars. The other discusses the different animation authoring paradigms and how Deimos uses them. We hope that these discussion points increases the contribution to knowledge/theory of our work, as they may help guide and influence future work on animated transitions---especially in Immersive Analytics.

Lastly, the following are the miscellaneous changes made to the manuscript:
- We fixed several typos as pointed out by R1 and R2, alongside several others (not highlighted).
- We replaced the term "mixed reality" with "augmented reality" as the latter is more commonly used.
- We changed the layout of Figure 5 so that it is hopefully easier to read and understand (R1).
- We increased the size of the code in Figure 8 (R2). While this does cause some lines to wrap around, this is a worthwhile trade-off.
- We changed all images to PDF format to allow text to be selected and copied.


==> Letter_to_Reviewers_2.tex <==
Dear ACs,

We have made changes to the manuscript with respect to the three dot points listed in the 1AC's re-review.

We added more justification to Section 4.4 as per R3's suggestion, by reiterating the possibility of a GUI being developed on top of the proposed Deimos grammar. The use of the desktop to author morphs is a fundamental choice made in this work, as jumping straight to designing a GUI would have been premature in our opinion.

We are not sure what R1 means by keeping the research questions in, as these were not present in the initial submission of our manuscript. Nevertheless, we have adjusted our list of contributions in Section 1 as per R1 and R2's suggestions. In particular, we condensed the engineering contributions together, and added new contributions which focus on the contribution to knowledge. One of these directly stems from a suggestion made by R2 in the first round of reviews which we greatly appreciate.

Lastly, we slightly tweaked the last paragraph of Section 2.1 to be less vague and link to Section 3 which does cover the differences with respect to prior work. We believe and hope that the updated list of contributions in Section 1 should resolve any remaining issues regarding the (lack of) contribution to knowledge in the first and second submissions.

==> original-sections/0._abstract.tex <==
\begin{abstract}
We present Deimos, a grammar for specifying dynamic embodied immersive visualisation morphs and transitions. A morph is a collection of animated transitions that are dynamically applied to immersive visualisations at runtime and is conceptually modelled as a state machine. It is comprised of state, transition, and signal specifications.
States in a morph are used to generate animation keyframes, with transitions connecting two states together. A transition is controlled by signals, which are composable data streams that can be used to enable embodied interaction techniques. Morphs allow immersive representations of data to transform and change shape through user interaction, facilitating the embodied cognition process.
We demonstrate the expressivity of Deimos in an example gallery and evaluate its usability in an expert user study of six immersive analytics researchers. Participants found the grammar to be powerful and expressive, and showed interest in drawing upon Deimos’ concepts and ideas in their own research.
%We demonstrate the use of Deimos in a gallery of diverse examples. We then evaluated the grammar and its concepts in an expert user study involving six fellow immersive analytics researchers. Participants used the toolkit unsupervised and were interviewd  and were interviewed for their thoughts and opinions afterwards.
\end{abstract}

==> original-sections/1._introduction.tex <==
\section{Introduction} \label{sec: introduction}
%In distributed cognition theory cognitive phenomena are considered a system involving not only a person’s internal representation of the world, but a system of translation and coordination of representations between internal and external representations, actors, and artefacts.
%Transformations of representations of information are considered key to cognition.  As we learn about information that we see in the world, we internalise this information by building conceptual models.  As these grow too large for us to process in short-term memory, we externalise them again with representations in the world, and we transform our external representations to gain different perspectives.  The role of distributed cognition as a theoretical framework for information visualisation, and the important role that interaction and transformation of representations plays in visualisation, has been considered by Liu et al.~\cite{liu2008dcog}.

%Within distributed cognition, the theory of Embodied Cognition suggests that human beings make sense of the world through our interaction with it \cite{gibbs2005}.  These interactions between our bodies and tools and the objects around us embody our dynamic reasoning process in a continuous interplay that is far richer than a static representation, such as a traditional chart or other data visualisation.  Immersive environments such as virtual and mixed reality (VR/MR) give human beings a platform for human computer interaction that has far greater potential for utilising a variety of human senses and the full range of physical human interaction capability.  Furthermore, as explored recently by Lee et al.\ \cite{leeDesignSpaceData2022}, immersive environments give us the freedom to move representations of information freely between two and three-dimensional forms as necessary, to either optimally project or spread information without occlusion across surfaces, or to faithfully represent 3D spatial data in the space around us.

%However, compared to the decades that have been invested in developing screen-based representation and interaction, tools for immersive data representation and interaction lag far behind.  Furthermore, prior to this paper, the existing frameworks for data visualisation in immersive environments have focused on static representation of the data in the environment.
%Past tools have not, however, given focus to transformations of data representations in a way that seems essential to support embodied cognition.  In sum, tools for authoring embodied interaction with data lag behind tools for authoring static representations.  

Within distributed cognition~\cite{liu2008dcog}, the theory of Embodied Cognition suggests that human beings make sense of the world through our interaction with it \cite{gibbs2005}. These interactions between our bodies and tools and the objects around us embody our dynamic reasoning process in a continuous interplay that is far richer than a static representation, such as a traditional chart or other data visualisation.  Immersive environments such as virtual and mixed reality (VR/MR) give human-beings a platform for human computer interaction that has far greater potential for utilising a variety of human senses and the full range of physical human interaction capability.  Furthermore, as explored recently by Lee et al.\ \cite{leeDesignSpaceData2022}, immersive environments give us the freedom to move representations of information freely between two and three-dimensional forms as necessary, to either optimally project or spread information without occlusion across surfaces, or to faithfully represent 3D spatial data in the space around us.

However, compared to the decades that have been invested in developing screen-based representation and interaction, tools for immersive data representation and interaction lag far behind.  Furthermore, prior to this paper, the existing frameworks and tools for data visualisation in immersive environments have focused on static representation of the data in the environment.
These frameworks and tools have not given attention to transformations of data representations in a way that seems essential to support embodied cognition.  In sum, tools for authoring embodied interaction with data lag behind tools for authoring static representations in immersive environments.

Therefore, in this paper we introduce Deimos: a declarative grammar for authoring \textbf{d}ynamic \textbf{e}mbodied \textbf{i}mmersive \textbf{mo}rph\textbf{s} for immersive visualisations. In contrast to traditional animated transitions, morphs are \textit{adaptive} and can be applied to any data visualisation in the environment that matches the partial visualisation specification of one of the morph's \textit{states}. \textit{Transitions} connect these states together to enable the actual animation, and can be controlled by \textit{signals}: data streams which stem from \textit{embodied} user interaction. These are specified using the Deimos grammar and are written in JSON.
 
We begin by detailing a set of design goals which allow immersive transitions to leverage the strengths of immersive environments that are not present on desktops~(Section \ref{sec: design-goals}). We then introduce the Deimos grammar itself, detailing its components, primitives, and specification (Section~\ref{sec: grammar}). Next, we describe a prototype implementation of the Deimos grammar (Section~\ref{sec: prototype}), developed in Unity as an extension to the DXR~\cite{sicatDXRToolkitBuilding2019} toolkit by Sicat et al. To demonstrate the expressivity of Deimos, we present an example gallery of morphs created in Deimos which highlight key characteristics of the grammar (Section~\ref{sec: example-gallery}). We also conducted a user study in which six immersive analytics researchers used Deimos to create their own morphs. We held a semi-structured interview with these participants in order to gauge the usability of Deimos (Section~\ref{sec: user-study}), as well as to elicit discussion topics and future research directions of immersive animated transitions (Section~\ref{sec: discussion}).


% !!! reverse this

% \begin{enumerate}
%     \item Animated transitions help to engage viewers and improve readability and transition awareness when presenting insights in data
%     \item Many grammars and toolkits have been developed to help designers create effective animated transitions on screens
%     \item With the growth of immersive analytics, it is natural to then consider the use of animated transition in immersive environments.
%     \item While there exist many instantiations of immersive analytics systems and toolkits, none directly address or consider the use of animated transitions.
%     \item Moreover, the shift to immersive is far more complex than just the addition of the third dimension, and thus warrants detailed consideration.
%     \item In this work, we explore the use of animated transitions in immersive environments by devising a grammar in which they can be defined
% \end{enumerate}

% Immersive visualisations are embodied interactions which itself can morph, change shape, etc.
% Put a use case here in order to establish the context and paint a picture to the user
% In short, front load a lot of the key differences as possible (section 3)




==> original-sections/2._related-work.tex <==
\section{Related Work} \label{sec: related-work}
\subsection{2D Animated Transitions}
When a visualisation changes between visual states, it is common to use animation to maintain transition awareness~\cite{heerAnimatedTransitionsStatistical2007}. Various animated transition grammars have been developed to allow designers to easily design and create 2D animated statistical graphics for use in data storytelling, such as Gemini~\cite{kimGeminiGrammarRecommender2021} and Gemini{\textsuperscript{2}}~\cite{kimGeminiGeneratingKeyframeOriented2021}, Canis~\cite{geCanisHighLevel2020} and CAST~\cite{geCASTAuthoringDataDriven2021}, and DataAnimator~\cite{thompsonDataAnimatorAuthoring2021}. While they each operate in different ways, they all functionally use keyframe animation, which has been shown to be the most preferred paradigm by animation designers~\cite{thompsonUnderstandingDesignSpace2020}. Earlier work by Tversky et al.~\cite{tverskyAnimationCanIt2002} however has suggested that interactivity may be needed to capitalise on the strengths of animation --- an area not properly explored in the aforementioned grammars. Indeed, research has found that interactive animation can improve outcomes for certain data analysis tasks (e.g., \cite{robertsonEffectivenessAnimationTrend2008, abukhodairDoesInteractivityImprove2013}). Recent work by Zong and Pollock et al.~\cite{zongAnimatedVegaLite2022} has sought to formalise this in the form of Animated Vega-Lite, an extension to Vega-Lite~\cite{satyanarayanVegaLiteGrammarInteractive2017} which adds a time encoding channel and event streams to enable interactive animations for use in data analysis. While our work also aims to combine interactivity and animation together, ours is clearly distinguished from Zong and Pollock et al.~\cite{zongAnimatedVegaLite2022} by its immersive nature. As immersive environments face new challenges and opportunities for how such interactive animations can behave, this work takes a fundamentally different approach to that of prior work in 2D animated transitions.

\subsection{Embodied, Immersive Analytics Tools and Toolkits}
Embodiment and animated transitions have been introduced in recent immersive visualisation research. In both ImAxes~\cite{cordeil2017imaxes} and its tangible version using the MADE-Axis~\cite{smileyMadeAxisModular2021}, embodied interaction is used to build visualisations, but this interaction is limited to authoring and does not support animated transitions into other visualisations. DataHop~\cite{hayatpur2020datahop} makes judicious use of animation to seamlessly transition between different configurations of data visualisations during exploration, but the use of animation was not a focus of their work. Similarly, tools like Flow Immersive~\cite{flowImmersive} also use animations to support transitions between visualisations, but are primarily used in data storytelling contexts.

In recent years, many toolkits and frameworks have emerged to support research and development in Immersive Analytics. Some specialised frameworks have been developed which focus on specific application cases. MIRIA~\cite{buschel2021miria} allows user experiment data such as head and hand movements to be replayed in a MR environment for in-situ analytics. However, the animations in the toolkit are limited to playing back user traces.
RagRug~\cite{fleckRagRugToolkitSituated2022} is a situated analytics toolkit that updates immersive visualisations in MR through the use of a distributed data flow from the Internet of Things. However, their work does not focus on embodied interaction to interact with situated visualisations, let alone animated transitions.
More broadly, toolkits like IATK~\cite{cordeilIATKImmersiveAnalytics2019}, DXR~\cite{sicatDXRToolkitBuilding2019}, VRIA~\cite{butcherVRIAWebBasedFramework2021}, and u2vis~\cite{reipschlager2020personal} have been developed to target immersive abstract visualisation scenarios. Those tools mainly provide authoring controls via a GUI or human-readable configuration files like JSON. In the case of DXR and VRIA, users control the design of visualisation objects using an implementation of the Vega-Lite grammar \cite{satyanarayanVegaLiteGrammarInteractive2017}.
Some toolkits also have built-in animations whenever data dimensions or visual attributes are changed, such as IATK~\cite{cordeilIATKImmersiveAnalytics2019}, but these are not designed to support more advanced animated transitions.

Recent work by Lee et al.~\cite{leeDesignSpaceData2022} remains one of few in Immersive Analytics which focus primarily on animated transitions. They present a design space for how immersive data visualisation transformations can be created, and present several examples and use cases. However, their work is conceptual in nature, and does not formalise in concrete terms how immersive animated transitions can be constructed. In this work, our aim is to create a grammar which allows users to construct and customise the behaviour of immersive transitions.

%RagRug \cite{fleckRagRugToolkitSituated2022}, is a situated analytics visualisation toolkit that allows the creation of visualisations with embodied interaction but the toolkit's data flow does not allow to explicitly define the embodied nature of  interaction itself and does not support morphs. Reipschlager et al \cite{reipschlager2020personal} introduced u2vis, a framework to support immersive visualisation for personal visualisation and interaction in mixed reality and wall-sized displays, but did not support continuous animated transitions. Lee et al. \cite{leeDesignSpaceData2022} have developed a framework to support immersive transitions with embodied interactions, but did not introduce a formal implementation to design such transitions. 




% \begin{enumerate}
%     \item Immersive analytics has been used for many purposes...
%     \item Existing research has explored how these can be used to offer engaging visualisations and interactions...
%     \item Several works have democratised the creation of immersive visualisation in the form of toolkits...
%     \item These vary in their approach, both in terms of grammar and in technical implementation
%     \item In our work, we decide to leverage DxR due to its Vega inspired syntax
%     \item The gap: no toolkit include high level design of interactive systems that support fluid transitions for data exploration (cite Niklas' paper Fluid interaction)
%     \item data (and visualisations) transformations to support sensemaking
% \end{enumerate}


% \subsection{Animated Transitions in 3D Environments}
% \begin{enumerate}
%     \item Works specifically addressing animated transitions in immersive environments are limited...
%     \item Some work has used animated transitions in its pursuit of other goals...
%     \item The most recent work of this is the CHI paper...
%     \item Therefore, this work draws inspiration from said work as its core concepts
% \end{enumerate}

==> original-sections/3._design-goals.tex <==
\section{Deimos Design Goals} \label{sec: design-goals}
The shift from 2D to 3D is more than just a third spatial encoding. Early on in the development of Deimos, we identified several key differences between animated transitions in immersive and non-immersive environments. We synthesised these into design goals (DG) which then influenced the creation of the Deimos grammar, allowing us to focus on the novel characteristics of immersive headsets and environments, in turn opening up further design opportunities.

\subsection{DG1: Immersive transitions be adaptable and flexible.}
Most animated transition grammars allow for rapid prototyping between the specification and the resulting animation. A low viscosity authoring process is particularly important when creating interactive animations for data analysis~\cite{zongAnimatedVegaLite2022}, allowing for fast and easy changes in the specification. The ability to rapidly prototype is facilitated by the constant access of keyboards for text input and pointing devices (i.e., mice) on desktop environments. In contrast, immersive environments often lack a convenient and comfortable form of text input that is required to write textual specifications, especially in VR or in highly mobile and/or remote MR contexts. While a GUI can help facilitate this authoring process in VR/MR, designing a GUI is premature if there is no underlying grammar to support it, especially in such a novel environment.

To resolve this conflict, we take an approach inspired by Lee et al.'s recent work~\cite{leeDesignSpaceData2022}. Many animated transition grammars treat transitions as a bespoke set of changes applied to visualisations predefined by the animation designer. Instead, we treat animated transitions as discrete operations that analysts can use to apply changes to their visualisations during their analysis. For example, the analyst might apply an animated transition which adds another spatial encoding to their visualisation, or converts a 3D barchart into a faceted 2D barchart. This turns animated transitions into a catalogue of adaptive and flexible operations that can be applied to immersive visualisations by analysts depending on the situation and goals.
In this way, there exists two types of users of Deimos: immersive analytics system designers who use the grammar to create a catalogue of animated transitions in a desktop environment (e.g., Unity editor), and data analysts in VR/MR who use said animated transitions in their workflows and either don't have access to or are unfamiliar with the grammar.
This necessitates a functional shift in grammar design, moving from highly tailored transitions with known data fields and encodings to generic transitions that operate on baseline idioms. As a result, any given transition specification can be reused across multiple visualisations, so long as they meet the baseline criteria specified by the author (e.g., be a barchart, have no \textit{z} encoding).


% Most animated transition grammars, when used for data analysis, rely on rapid prototyping between the specification and resulting (interactive) visualisation \cite{zongAnimatedVegaLite2022}. This is possible due to the near ubiquitous access to keyboards for symbolic input on desktop environments. This is not always the case for immersive environments, such as in virtual reality or in highly mobile and remote contexts. While a GUI can overcome this shortcoming, this is premature if there is no underlying grammar to support it, especially in such a novel environment. Therefore, in a similar vein to recent work by Lee at al.~\cite{leeDesignSpaceData2022}, we treat animated transitions as discrete operations usable during data exploration, augmenting any existing authoring tools or processes. Traditionally, bespoke transition specifications are written for every visualisation. Instead, we envision a catalogue of transition specifications being applied dynamically to any applicable visualisations in the immersive scene. 
% In this way, animated transitions can essentially be pre-made for end-users who either don't have access to or are unfamiliar with the grammar. This necessitates a functional shift in grammar design, moving from highly tailored transitions with known variables and encodings to generalised transitions that operate on baseline idioms. As a result, any given transition specification can be reused across multiple visualisations, so long as they meet the baseline criteria specified by the author (e.g., be a barchart, have no \textit{z} encoding).

\subsection{DG2: Immersive transitions should leverage embodied interaction}
Animated transition grammars (e.g., \cite{kimGeminiGrammarRecommender2021, geCanisHighLevel2020, thompsonDataAnimatorAuthoring2021}) have paid little attention to how transitions are triggered and controlled. In cases where these grammars do (e.g., \cite{zongAnimatedVegaLite2022}) it is limited to WIMP-style controls, with practitioners using similar input methods for their narrative visualisations (e.g., play button~\cite{roslingGapminder2007}, linear slider/scroll~\cite{yeeR2d3}).
In contrast, immersive environments rely on a completely different interaction paradigm which goes beyond the desktop and is both embodied (e.g.,~\cite{hurterFiberClaySculptingThree2019, cordeilIATKImmersiveAnalytics2019}) and spatial in nature (e.g.,~\cite{hubenschmidSTREAMExploringCombination2021, buschelInvestigatingUseSpatial2017}).
Novel language primitives are needed for this as existing ones (i.e., streams in \cite{zongAnimatedVegaLite2022}) do not adequately express relationships between entities, such the direct manipulation of user actions onto target objects (e.g., controller inputs on visualisations~\cite{hurterFiberClaySculptingThree2019}) or the spatial relationship between multiple objects in the immersive environment (e.g., position and orientation of a handheld in relation to a table~\cite{buschelInvestigatingUseSpatial2017}).
%Animated transition grammars typically focus on customising the behaviour of the animation (e.g., staging, staggering), paying little attention to how the overall transition is both triggered and controlled in the first place (e.g., \cite{kimGeminiGrammarRecommender2021, geCanisHighLevel2020, zongAnimatedVegaLite2022}). Wherever there is interactivity, they tend to use WIMP-style controls such as a binary ``play'' button (e.g., Gapminder~\cite{roslingGapminder2007}) or one-dimensional input using via slider or scroll (e.g., R2D3~\cite{yeeR2d3}). 
%In contrast, immersive environments afford a wider range of input modalities and techniques, including embodied (e.g.,~\cite{hurterFiberClaySculptingThree2019, cordeilIATKImmersiveAnalytics2019}) and spatial interaction (e.g.,~\cite{hubenschmidSTREAMExploringCombination2021, buschelInvestigatingUseSpatial2017}).
By expanding our grammar to support this paradigm, we enable a richer design space of visualisation transitions not otherwise possible on desktop environments, as they allow users to ``reach through'' and interact with their data in a more embodied and engaging manner~\cite{dourishWhereActionFoundations2001}.
\textit{Tilt Map} by Yang et al.~\cite{yangTiltMapInteractive2020} remains a prime example of this concept. As the user tilts the visualisation object, it transitions between a choropleth map, prism map, and barchart at set angular intervals. These intervals are chosen such that the visualisation object is at an optimal viewing angle for each of the three states. Lee et al.~\cite{leeDesignSpaceData2022} also demonstrated numerous other examples of embodied interaction used to enable animated transitions, with the input action (e.g., pinch and drag gesture on visualisation) directly matching the resulting visual changes (e.g., additional dimension being extruded). We want our grammar to support these scenarios and more.


% \subsection{DG2: Immersive transitions should leverage embodied interaction}
% Animated transition grammars typically focus on customising the behaviour of the animation (e.g., staging, staggering), paying little attention to how the overall transition is both triggered and controlled in the first place \cite{zongAnimatedVegaLite2022}. Wherever there is interactivity, they tend to use WIMP-style controls such as a binary ``play'' button (e.g., Gapminder~\cite{roslingGapminder2007}) or one-dimensional input using via slider or scroll (e.g., R2D3~\cite{yeeR2d3}). 
% In contrast, immersive environments afford a wider range of input modalities and techniques, including embodied (e.g.,~\cite{hurterFiberClaySculptingThree2019, cordeilIATKImmersiveAnalytics2019}) and spatial interaction (e.g.,~\cite{hubenschmidSTREAMExploringCombination2021, buschelInvestigatingUseSpatial2017}). By expanding our grammar to support these, we enable a richer design space of visualisation transitions not otherwise possible on desktop environments. Tilt Map by Yang et al.~\cite{yangTiltMapInteractive2020} remains a prime example of this concept, with Lee et al.~\cite{leeDesignSpaceData2022} demonstrating numerous other examples of embodied interaction used to enable visualisation transitions. We want our grammar to support these scenarios and more.


\subsection{DG3: Immersive transitions should still support conventional approaches}
While the two previous design goals were intentionally forward thinking, we still want Deimos to be rooted in the same foundational elements as existing grammars. This is to both ensure that Deimos follows tried and true concepts and theories, and also to preserve a sense of familiarity for users of the grammar --- especially for those new to immersive analytics. This includes the use of keyframe animation as the chief animation paradigm~\cite{thompsonDataAnimatorAuthoring2021}, the ability to specify timing and staging rules to customise the animation, and supporting WIMP-based interaction in hybrid immersive analytics setups or via immersive UX elements (e.g.,~\cite{microsoftMixedRealityUX}).
Moreover, while DG1 advocates for generalised transitions that can be applied to a wide range of visualisations, Deimos should still allow for highly customised transitions that affect predefined visualisations created by designers. This is to allow animated transitions in Deimos to still be useful in controlled situations such as immersive data-driven storytelling.
Therefore, our grammar should support both ends of two orthogonal spectrums: support both WIMP and embodied interaction to control and interact with animated transitions; and support animated transitions that are either highly generalised and can apply to any visualisation, or highly specific and apply only to a particular visualisation in a controlled context.


% \subsection{DG3: Immersive transitions should still support conventional approaches}
% Despite the prior two principles, our grammar should still resemble that of existing grammars so as to not be wholly unfamiliar. This includes the use of keyframe animation as the choice of authoring paradigm~\cite{thompsonUnderstandingDesignSpace2020}, and supporting WIMP-based interaction in hybrid immersive analytics configurations and/or immersive UX elements (e.g.,~\cite{microsoftMixedRealityUX}). Moreover, having highly customised transitions can still be desirable in immersive environments, such as in immersive data-driven storytelling. Therefore, our grammar should support both ends of both spectrums: support both WIMP and embodied interaction to control transitions, and affect visualisations using both generalised and customised levels of specificity. Even so, it is important to stress that our goal is not to fully re-implement existing grammars such as Gemini~\cite{kimGeminiGrammarRecommender2021} and Canis~\cite{geCanisHighLevel2020}, but explore the unique characteristics of what a similar grammar might be like in immersive environments.

==> original-sections/4._grammar.tex <==
\section{The Deimos Grammar} \label{sec: grammar}
Deimos is a declarative grammar used to specify \textit{transitions} between \textit{states} (keyframes), as well as the \textit{signals} (interactions) used to control them. The grammar is largely based around the aforementioned design goals (Section~\ref{sec: design-goals}) and prior work by Lee et al.~\cite{leeDesignSpaceData2022}. The target audience of the grammar are developers and designers of immersive analytics systems. The animated transitions they create are then used by analysts in VR/MR. A Deimos specification can formally be described as a three-tuple (elements suffixed with ``?'' are optional):

\begin{center}
\textit{Morph := (states, signals?, transitions)}
\end{center}

These components constitute what we call a \textit{Morph}, the term signifying a visualisation's ability to dynamically change shape and morph from one state to another via transitions upon matching certain conditions. 
A morph can be modelled as a state machine (see Figure~\ref{fig:deimos-state-machine-1}). A visualisation in the immersive environment only enters a morph's state machine when it matches one of its \textit{states}. The state node that was matched with determines the possible \textit{transition} nodes that it can access. These transition nodes are where changes are actually made to the visualisation, and are only entered when specified criteria are met. These criteria take the form of \textit{signals}, which are streams of data typically generated by user interaction. They can also be used to control the behaviour of transitions themselves. 
%Multiple states and transitions can be composed together to form more complex morphs (see Figure~\ref{fig:deimos-state-machine-2}).

\begin{figure}[tb]
    \centering
    \includegraphics[width=7.5cm]{images/deimos-state-machine.pdf}
    \caption{Baseline state machine for Deimos morphs showing a single unidirectional transition. More states and transitions can be added to the state machine with their own signal criteria, with support for bidirectional transitions.}
    \Description{A state machine for a baseline morph. A node labelled ``State 1'' is connected with a directed edge to a node labelled ``Transition'', and is labelled with ``Signal criteria met''. The latter node is connected with another directed edge to another node labelled ``State 2'', and is labelled with ``Transition completed''. Two entry nodes connect to the two State nodes with labels reading ``State matched''. The two State nodes are also connected to an exit node reading ``Vis spec manually changed''.}
    \label{fig:deimos-state-machine-1}
\end{figure}


Morphs are an extension to any immersive visualisation authoring system already in place. That is, visualisations can still be manipulated in their usual way, but can have morphs applied to them should the relevant conditions be met. In this way, morphs serve purely to augment existing authoring techniques rather than supplanting them outright. When a visualisation is modified by the user in a manner external from the morph, it exits the morph state machine. It may then immediately re-enter following the same rules as before. A visualisation can have multiple morphs (and therefore state machines) active simultaneously. Multiple morphs can also be applied to the same visualisation concurrently, so long as the properties and encodings they affect do not overlap. The same morph specification can also be active across multiple eligible visualisations. This ability for the state machine to adapt to different visualisation configurations through a set of rules and conditions is what helps it satisfy DG1.

Morph specifications are written and stored as standalone JSON files. The use of JSON is very common amongst related grammars and allows for the separation between grammar and implementation (i.e., portability). A JSON schema provides auto-completion and tooltips for writing morph specifications with supported text editors. Figure~\ref{fig:deimos-json} shows a basic example of a morph specification, and how it translates to the immersive environment and the state machine. The three main components of morphs are annotated with coloured boxes: states in yellow, signals in blue, and transitions in green. The same colour-coding is used across all other figures.
The rest of this section will explain in general terms what these components do.

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{images/deimos-json.pdf}
    \caption{A basic example of a morph changes the mark colour of uncoloured visualisations to red whenever the left hand performs a pinch gesture. Colour-coded boxes denote the same component in different representations. Left: The morph specification. Top right: Still images of this morph being applied to a 2D scatterplot in an immersive environment. Bottom right: The state machine for this morph. The \texttt{``restrict'': true} (shown in the left-hand box labelled with ``2'') prevents the morph from starting at the \textit{highlighted} state, and \texttt{``bidirectional'': true} (shown at the end of morph specification) allows the transition to function in both directions.}
    \Description{An image composed of three parts. The first part shows a morph specification written in JSON. The second part shows a series of still images in which a hand does a pinch gesture, and causes the marks on a 2D scatterplot to turn red. The second part shows the state machine of this morph. The following three nodes are connected in a linear order: a ``unhighlighted'' state node, a ``highlighting'' transition node, and a ``highlighted'' state node.}
    \label{fig:deimos-json}
\end{figure}


\subsection{States} \label{ssc: states}
A morph is comprised of at least two state specifications. A state can be defined by the following tuple:

\begin{center}
\textit{state := (name, restrict?, partial visualisation specification)}
\end{center}


The \textit{name} property is a unique case-sensitive string used to reference this state specification in a transition (see Section~\ref{ssc: transitions}).
%The \textit{name} component is a unique case-sensitive string used to reference this state specification in a transition (see Section~\ref{ssc: transitions}).
The \textit{restrict} property is a Boolean that if set to \texttt{true} will remove the entry point associated with the state's node on the state machine (see Figure~\ref{fig:deimos-json} for an example). This prevents a morph from starting at that state, making it only accessible via interconnecting transition(s). This is useful if it is illogical for a morph to start at that state, such as in unidirectional transitions.
%The \textit{restrict} component is a boolean that, if set to \texttt{true}, will remove the entry point associated with this state's node on the Morph state machine (see Figure~\ref{fig:deimos-state-machine}). This means that the state is only accessible via an interconnecting transition --- useful when starting a morph at said state is illogical, such as in unidirectional transitions.
\textit{Partial visualisation specification} is an arbitrary number of properties and components in the state object that all follow the same declarative notation as an actual visualisation. In other words, its syntax is the same as the visualisation package used in the system. For our implementation of Deimos, this is the DXR grammar~\cite{sicatDXRToolkitBuilding2019} which in turn is based on the Vega-Lite grammar~\cite{satyanarayanVegaLiteGrammarInteractive2017}. In the context of the DXR grammar, a partial specification can consist of any number of view-level properties (e.g., \textit{mark}, \textit{depth}) and/or encoding-level properties declared inside of an \textit{encoding} component (e.g., \textit{x}, \textit{color}).
The partial specification serves two purposes: i) to determine if a visualisation matches (and therefore enters) this state; and ii) to generate the keyframe used in the transition.
%The \textit{partial visualisation specification} component is actually an arbitrary number of individual JSON properties of variable length (denoted by the ``\&''), and forms the bulk of the state specification. It serves two purposes: i) to determine if a visualisation matches (and therefore enters) this state; and ii) to generate the keyframe used in the transition. This component is fundamentally a portion or entirety of a declarative visualisation specification. The actual syntax used for this is dependent on the visualisation package used in the immersive analytics system. In the case of our implementation of Deimos, this is the DXR visualisation grammar~\cite{sicatDXRToolkitBuilding2019} which in turn is based on the Vega-Lite grammar~\cite{satyanarayanDeclarativeInteractionDesign2014}.

\subsubsection{State matching process} \label{sss: state-matching-process}
Any visualisation properties specified as part of the \textit{partial visualisation specification} in a state are used in the matching process against active visualisations. It is important to differentiate between the two types of specifications being used in this process: the visualisation specification created by the end-user, and the state specification (i.e., the \textit{partial visualisation specification}) that exists as a part of the state component in a morph.
Generally speaking, for a state specification to be matched against a visualisation specification, all properties defined in the former should also be defined in the latter, including their associated values. For example, if the state has \texttt{``color'': \{ ``type'': ``quantitative''\}}, then the visualisation must also have a \texttt{color} encoding with the same \texttt{type} for it to match.
\chreplaced{As a rule of thumb, the fewer properties defined in the state specification, the more likely a visualisation can match successfully and have morphs applied to it. The opposite is also true, with more properties in the state specification making it less likely for any visualisation to match successfully.}{As a rule of thumb, the less properties defined in the state specification, the more likely any given visualisation specification can successfully match against it and have morphs applied to and vice versa.} This effectively forms a spectrum. Morphs can be highly generic and can apply to many visualisations, allowing for adaptive morphs as per DG1. They can also only apply to specific datasets and field names, allowing for highly tailored morphs that are used in controlled environments as per DG3.
%This fulfils half of DG3.

Deimos provides several primitives which affect the matching process that can be used in place of any JSON value in the state specification. They allow for more nuanced control over which visualisations can and can't match, and are useful to prevent morphs from being accidentally applied to incompatible visualisations.
Note that this is not an exhaustive set of primitives. While they were adequate for the purposes of this work, the grammar can easily be extended to include more if need be.
%Deimos provides several primitives for more nuanced control over this matching process that can be used as values in the state specification:

\begin{itemize}
    \item \textbf{``*'' (wildcard)}: The property should be in the visualisation but its value can be anything.
    \item \textbf{An inequality expression}: The property should be in the visualisation and its value should satisfy the inequality. Only applicable to numeric properties. e.g., \texttt{``value'': ``>= 100''}.
    \item \textbf{\texttt{null}}: The property should not be included in the visualisation regardless of its value.
\end{itemize}

\subsubsection{Keyframe creation process} \label{sss: keyframe-creation-process}
When a visualisation matches a state and one of its connecting transitions is activated, keyframes are generated for both initial and final states. These keyframes are used for actual animation during the transition.
The initial keyframe is always the active visualisation's specification prior to the transition. No changes need to be made to it as it already matches the properties of the state itself.
The final keyframe is created by modifying the initial keyframe using the following set of rules: (i) visualisation properties that are defined in the initial state but not in the final state are removed; (ii) properties that are not defined in the initial state but are defined in the final state are added; and (iii) properties defined in both states are set to the final state's value.

As with the state machine process (Section~\ref{sss: state-matching-process}), Deimos provides primitives that can be used in place of any JSON value to refine the keyframe creation process. These primitives functionally act as placeholders which are later substituted with real values calculated at runtime, akin to the notion of variables. This allows for morphs to adapt to a wider range of situations without the need to hard-code field names, data types, etc. in morph specifications.
For the purposes of the state matching process, all of these primitives are treated as wildcards. Their values are resolved after the keyframes have been created but before the transition is applied. Once again, this is not an exhaustive list of primitives and can easily be extended if need be. 

\begin{itemize}
    \item \textbf{JSON path accessor}: The value residing at the JSON path will be substituted into the property's value. Is either prefixed with ``this.'' to access a property from this keyframe, or ``other'' to access a property from the other keyframe which is being transitioned to/from. e.g., \texttt{``x'': ``this.\linebreak[0]encoding.\linebreak[0]y'', \texttt{``field'': ``this.\linebreak[0]encoding.\linebreak[0]size.\linebreak[0]field''}}.
    \item \textbf{A signal name}: The value emitted by the specified signal (see Section~\ref{ssc: signals}) will be substituted into the property's value.
    \item \textbf{An expression}: The evaluated result of the expression will be substituted into the property's value. JSON path accessors and signal names can be used as variables. Only applicable to numeric properties. e.g., \texttt{``value'': ``other.\linebreak[0]encoding.\linebreak[0]size.\linebreak[0]value * 10''}.
\end{itemize}

All keyframes are stored throughout the entire lifespan of a morph. When the morph exits the state machine --- the result of the associated visualisation having its specification manually changed by the user (see Figure~\ref{fig:deimos-state-machine-1}) --- all stored keyframes are deleted. %and are deleted when the state machine exits.
Any added or changed properties will take their values from the state's keyframe if one already exists. 
The main purpose for this is to handle situations where a property is removed by a transition in one direction, but needs to be added back in by a transition in the reverse direction. Without stored keyframes, the removed property would no longer be known and therefore could not be added back in. 


\subsection{Signals} \label{ssc: signals}
In Deimos, a signal is the resulting value from a stream of data captured from input events, drawing inspiration from Vega's signals~\cite{satyanarayanDeclarativeInteractionDesign2014} and event-driven functional reactive programming principles~\cite{wanEventDrivenFRP2002}. Signals can be used in Deimos to: (i) be substituted as values in keyframes (see Section~\ref{sss: keyframe-creation-process}); (ii) act as conditional triggers that control when a transition actually begins (see Section~\ref{ssc: transitions}); and (iii) act as a tweening variable to control the progression of a transition (see Section~\ref{ssc: transitions}). No type safety is enforced in Deimos. A morph may contain zero or more signal specifications.
Deimos has two main types of signals: signals that stem from some given source, and signals that evaluate a mathematical expression. 

\begin{center}
    \textit{signal := sourceBasedSignal | expressionSignal}
\end{center}


\subsubsection{Source-based Signals} \label{sss: source-based-signals}
Source-based signals, as the name suggests, emit values from some input source. This is primarily from user interactions, but could be extended to passively updating values from sensors, etc. We define two classes of source-based signals: deictic and non-deictic signals. Deictic signals express relationships between a source and target entity.
While they mainly serve to model direct manipulation which is commonly associated with embodied interaction (DG2), they can also model situations where there is no actual direct contact. Non-deictic signals capture everything else, although these are mainly input sources which do not require some target/context to make sense (e.g., mid-air hand gestures, input source states, sensor data). Their production rules are:

\begin{center}
\begin{tabular}{l}
    \textit{sourceBasedSignal := nonDeicticSignal | deicticSignal} \\
    \textit{nonDeicticSignal := (name, source, handedness?, value)} \\
    \textit{deicticSignal := (name, source, handedness?, target, criteria?, value)}
\end{tabular}
\end{center}

Both signal classes share the same three attributes.
The \textit{name} property references this signal in either a state (see Section~\ref{sss: keyframe-creation-process}), an expression signal (see Section~\ref{sss: expression-signals}), or a transition (see Section~\ref{ssc: transitions}).
The \textit{source} property denotes the type of source that values are to be retrieved from (e.g., \texttt{hand}, \texttt{head}, \texttt{vis}, \texttt{ui}).
Certain sources can also specify the source's \textit{handedness} to distinguish between \texttt{left}, \texttt{right}, or defaulting to \texttt{any}.

%Both signal classes share the same three components. The \textit{name} component is a unique case-sensitive string used to reference this signal in either a state (see Section~\ref{sss: keyframe-creation-process}), an expression signal (see Section~\ref{sss: expression-signals}), or a transition (see Section~\ref{ssc: transitions}).
%The \textit{source} component denotes the type of source that values are to be retrieved from (e.g., \texttt{hand}, \texttt{head}, \texttt{vis}, \texttt{ui}). Certain sources can also specify the source's \textit{handedness} to distinguish between left, right, or any, defaulting to \texttt{any}.

For non-deictic signals, the \textit{value} property denotes what type of value to derive from the source, which is then emitted by the signal. This can either be the state of the user interaction (e.g., whether the hand is performing a \texttt{select} gesture) or the geometric properties of the source as an object in the immersive environment (e.g., \texttt{position} of the user's head). As previously mentioned, these are useful to when some value of the input source is to be retrieved without it needing to be in the context of some other target or object. Figure~\ref{fig:deimos-json} shows an example of a non-deictic signal: it does not matter what the hand is touching so long as it is performing the pinch gesture.
%For non-deictic signals, the \textit{value} component denotes what type of value to derive from the source, which is then emitted by the signal. This can either be the the state of the user interaction (e.g., whether the hand is performing a \texttt{select} gesture) or the geometric properties of the source as an object in the immersive environment (e.g., \texttt{position} of the user's head). Specific to our implementation (see Section~\ref{sec: prototype}), .NET reflection can also be used to access values from the source GameObject in Unity (e.g., \texttt{transform.position.x} of the user's hand).

Deictic signals model relationships between entities, and are modelled closely after the interaction section of the design space by Lee et al.~\cite{leeDesignSpaceData2022}.
The \textit{target} property denotes the type of object that the source is attempting to target. This can either be a part of the visualisation (e.g., \texttt{mark}, \texttt{axis}), a separate object in the environment (e.g., \texttt{surface}), or part of the user themselves (e.g., \texttt{head}).
For the first two, a \textit{criteria} property needs to be included to determine the logic used in selecting the target (e.g., \texttt{select}, \texttt{touch}, \texttt{nearest}). This logic is needed when there are multiple potential target objects that could be selected.
Lastly, the \textit{value} property can be used to derive three types of values. First, it can derive values from the \textit{target} much in the same way as non-deictic signals do. For example, a \texttt{hand} source might target the \texttt{mark} that it is \texttt{select}ing, and the \texttt{position} of that mark is used as the value. Second, it can derive values from a comparison between the source and target. For example, a \texttt{vis} source might target the \texttt{surface} that it is \texttt{touch}ing, and the point of \texttt{intersection} between the vis and surface is used as the value. Third, a \texttt{boolean} value simply emits true if a target has been selected successfully, and false if no targets are selected.

Deictic signals in particular fulfil DG2 as they allow morphs to be controlled based on user input and the embodied objects in the environment which they interact with. Moreover, the ability to facilitate WIMP-style interaction using these signals also helps fulfil DG3.

%     \item Inspired by Vega, we use Signals in order to enable user control of Morphs
%     \item These signals can be used to modify the keyframes generated from the states (see above), used to act as conditions for when the transition should occur, and/or to control to progression of the transition (i.e., its tween). In this section we describe how the signals are created in the first place
%     \item Our signals take heavy inspiration from the CHI paper
%     \item We characterise these signals into three types: a) signals that do not target any specific element (also known as non-deictic signals); b) signals that target a specific element (known as deictic signals); and c) signals that are evaluated based off of a mathematical expression
%     \item Signals are typically a result of user input, but may also be passively updating variables as well
%     \item Note that as signals can produce data values of varying types, no type safety is enforced
%     \item As with states, all signals require a (unique) name


\subsubsection{Expression Signals} \label{sss: expression-signals}
\begin{center}
    \textit{expressionSignal := (name, expression)}
\end{center}

Expression signals allow for the arbitrary composition of signals using mathematical expressions. Their primary purpose is to modify and refine values emitted by source-based signals.
We choose to use expressions as they allow arbitrary calculations to be performed in a familiar manner, instead of designing a completely new and potentially confusing domain-specific language.
The \textit{name} property references this signal in the same way as source-based signals. The \textit{expression} property is a mathematical expression as a string. Basic mathematical operators can be used alongside select primitive functions (e.g., \texttt{normalise}, \texttt{distance}, \texttt{angle}).
As with all other primitives, the list of supported functions can easily be extended. Any type of signal can be used as a variable by referencing their name. As previously mentioned, no type safety is enforced, meaning the user has to be aware of the data types present in the expression.


\subsection{Transitions} \label{ssc: transitions}
A morph is comprised of at least one transition specification. They functionally connect two state specifications together in the state machine (see Figure~\ref{fig:deimos-state-machine-1}). A transition can be defined by the following seven-tuple:

\begin{center}
\textit{transition := (name, states, trigger?, control?, bidirectional?, disablegrab?, priority?)}
\end{center}

The \textit{name} property serves to identify this transition especially when multiple transitions are involved.
%The \textit{name} component is a unique case-sensitive string used by the system to identify each transition, but is not referenced in any other part of the grammar.
The \textit{states} property is an array of two strings, corresponding to the names of the initial and final states in the transition respectively. Referencing states via their name in this manner helps with encapsulation, keeping all state related syntax separated from the transitions.
%The \textit{states} component is an array of two strings, corresponding to the names of the initial and final states in the transition respectively.
The \textit{trigger} property is an equality expression that activates the transition when it evaluates as true, but only when the visualisation matches the initial state in the \textit{states} property. The expression follows similar rules as expression signals (see Section~\ref{sss: expression-signals}) but must return a Boolean value. Triggers are mainly used to let the user control when the transition is actually applied, usually as the result of some sort of input action or condition caused by the user. Not setting a trigger will cause the transition to be immediately applied when it enters the initial state.
%The \textit{trigger} component is an equality expression that activates the transition when it evaluates as true, but only when the visualisation matches the initial state in the \textit{states} component. The expression follows similar rules as expression signals (see Section~\ref{sss: expression-signals}) but must return a boolean value. Not setting a trigger will cause the transition to be immediately applied when it enters the initial state.

The \textit{control} component is optionally used to further customise the behaviour of the transition. It is formally described by the following five-tuple:

\begin{center}
\textit{control := (timing?, easing?, interrupted?, completed?, staging?)}
\end{center}

The \textit{timing} property controls the duration of the transition. If a number is used, the transition will interpolate between the two state keyframes over the given duration in seconds. Alternatively, the name of a signal can be used, in which case the signal will be used as the tweening variable \textit{t}. This allows for the duration and direction of the interpolation to be controlled by the signal (and subsequently the user). In this situation, the transition will only begin when the signal is a value between 0 and 1, in addition to any other conditions. This defaults to 0 if not specified, which will result in jump cuts.
The \textit{easing} property applies an easing function to the transition, defaulting to a linear function if none is specified. Easing functions are commonly used in animations and helps to make animations look more natural.
The \textit{interrupted} property determines what happens when the \textit{trigger} returns false whilst the transition is in progress. \texttt{initial} and \texttt{final} will cause the visualisation to immediately jump to the specified state. \texttt{ignore} will instead allow the transition to keep progressing until it naturally terminates. The \texttt{ignore} condition is particularly useful in cases where the \textit{trigger} may inadvertently return false mid-transition but the transition should still continue, acting as a sort of fail-safe. This defaults to \texttt{final}.
Similarly, the \textit{completed} property determines what happens when the visualisation naturally terminates, either remaining at the \texttt{final} state or resetting back to the \texttt{initial} state. Using the \texttt{initial} condition may be useful if the transition should not cause any long term changes to the visualisation, particularly if the animation is alone sufficient to serve its purpose~\cite{leeDesignSpaceData2022}. This also defaults to \texttt{final}.

The \textit{staging} property allows for specific visualisation properties to be staged. Name-value pairs can be specified where the name is the property to be staged, and value is an array of two numbers between 0 and 1 that correspond to start and end percentages. The property will only be animated when the transition period is within the given range. Any property not specified will not be staged. Staging is a common feature of animated transition grammars~\cite{heerAnimatedTransitionsStatistical2007} and ours is no different. Note that the grammar does not support staggering.

The \textit{bidirectional} property of the transition, if set to true (default false), allows the transition to start and end in the reverse direction. All transition settings remain the same, except the \textit{trigger}, if specified, needs to return false in order for the reverse transition to activate. This serves mainly as a convenience function which prevents the need for two transition specifications to be written whenever a single bidirectional transition is desired. However, doing so is necessary in order to have distinct settings for either direction.
The \textit{disablegrab} property, if set to true (default false), will automatically disable the standard VR/MR grab action performed on the visualisation when the transition starts. This helps prevent visualisations from being inadvertently moved by the user when a transition's \textit{trigger} uses a similar grab gesture.
Lastly, the \textit{priority} property can be used to handle edge cases where multiple transitions due to similar \textit{trigger} conditions are activating on the same frame, but they conflict in the visualisation properties they modify. In this situation, the transition with the highest numbered priority will activate first, and all other conflicting transitions will be blocked. If priorities are equal, then the order in which they activate is random. The priority property defaults to 0.


==> original-sections/5._prototype.tex <==
\section{Deimos Implementation and Toolkit} \label{sec: prototype}
We created a prototype implementation of the Deimos grammar using the Unity game engine in order to demonstrate its concepts and use. It is open source on a GitHub repository\footnote{Github link provided on acceptance. For review, the project files are instead provided in supplementary material.}, with documentation also available publicly\footnote{Link will be provided upon acceptance. For review, the documentation is instead provided in supplementary material}.

\subsection{Data Visualisations} \label{ssc: prototype-data-visualisations}
As Deimos is primarily an animated transition grammar, we need data visualisations to apply transitions to. We decided to use DXR~\cite{sicatDXRToolkitBuilding2019} as the basis of our work as it natively supports authoring of visualisations using a declarative grammar similar to Vega-Lite~\cite{satyanarayanVegaLiteGrammarInteractive2017}. It is also easy to extend due to its use of individual GameObjects for each mark instead of a single mesh for all marks like in IATK~\cite{cordeilIATKImmersiveAnalytics2019}. This came at the cost of rendering performance however, especially when thousands of marks are displayed on screen. To this end, we made performance improvements to how DXR instantiates and updates its marks and axes, especially since this process occurs multiple times in a morph.
We also added several new visualisation types: choropleth and prism maps, stacked and side-by-side barcharts, and faceted charts (see Section~\ref{sec: example-gallery}). However, as the original DXR implementation does not have support for data transformations like in Vega-Lite, neither does Deimos. This also means that animated transitions involving a time dimension (e.g., time varying scatterplots, barchart races) are not supported in Deimos.


\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{images/deimos-overview.pdf}
    \caption{Overview of Deimos and how it interacts with DXR. Recreated version of the original DXR overview~\cite{sicatDXRToolkitBuilding2019} is shown in the lower half.}
    \Description{A diagrammatic image Deimos. Deimos morph specifications connect to the Deimos package. User inputs also connect to the Deimos Package. Below it, a DXR vis specification connects to Data and the DXR package. The Deimos and DXR packages are connected to each other, with arrows indicating ``DXR vis updated'' and ``Start/stop transition''. The DXR package then connects to the Morphing DXR vis.}
    \label{fig:deimos-overview}
\end{figure}

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{images/deimos-pipeline.pdf}
    \caption{High-level overview of the Deimos pipeline. Stages in red signify events that cause Deimos to continue down the pipeline.}
    \Description{A linear flowchart of the Deimos pipeline. The nodes in linear order are Load morph specifications, DXR vis updated (in red), Find matching states, Create observables from signals, Trigger returns true (in red), Create keyframes, Start transition, Transition finished (in red), Stop transition, and Dispose observables. The last node is connected back to the Find matching states node.}
    \label{fig:deimos-pipeline}
\end{figure}

\subsection{Code Structure and Pipeline}
Figure~\ref{fig:deimos-overview} provides an overview of Deimos' structure and how it interacts with DXR.
Morph specifications are contained in JSON files that are read by Deimos at initialisation. They can also be refreshed during runtime if the specifications are edited. Deimos interacts with DXR in two main ways. Deimos receives events from DXR whenever a visualisation has been updated, which includes the visualisation specification as an argument. Deimos also sends start and stop function calls to DXR which executes the animated transitions.

Figure~\ref{fig:deimos-pipeline} provides a high-level overview of the Deimos pipeline. While it is presented as a linear set of stages, the pipeline can reset or be exited in certain conditions.
First, all morph specifications are read and loaded into Deimos.
Next, whenever a DXR visualisation updates, Deimos is notified via event with the visualisation's specification.
This specification is used to check against all state specifications in the loaded morphs using the rules in Section~\ref{sss: state-matching-process}.
For any state that has matched, observable streams are created for each signal that is part of the state's transitions, including trigger signals. Observables are created using the UniRx package~\cite{neueccUniRx}, and are composed together where necessary.
When a transition's trigger signal returns true (or if no trigger was specified in the first place), initial and final keyframes are created using the rules in Section~\ref{sss: keyframe-creation-process}.
These two keyframes, along with other transition parameters such as tweening and staging variables, are sent to the relevant DXR visualisation to start the transition.
When the transition has finished, Deimos stops the transition on the DXR visualisation. This step also updates the visualisation specification to reflect the new changes made by the transition.
Deimos then disposes of all observables related to the transition.
This process then starts anew again, with Deimos finding matching states to see if this newly updated visualisation is eligible for any morphs once more.

%Whenever a DXR visualisation is updated, Deimos evaluates its specification against the states in all loaded morph specifications. For each matching state, Deimos goes through its valid transitions, creating and subscribing to the data stream (see Section~\ref{ssc: prototype-signals}) for its trigger, which is usually based on data values from user inputs upstream (see Section~\ref{sss: source-based-signals}). When the stream emits true, Deimos creates two keyframes using the rules described in Section~\ref{sss: keyframe-creation-process}. These keyframes are essentially complete DXR visualisation specifications, one labelled as the initial and the other as the final keyframe. These, alongside other control variables (e.g., tweening stream, easing and staging values), are sent via function call to the relevant DXR visualisation to start the transition.
%If a transition is active and the stream emits false, or if the visualisation no longer matches the state, Deimos does a function call to DXR to stop the active transition.

While Deimos is designed such that it exists separately from the visualisation framework used, they are still intrinsically linked to each other. Deimos is dependent on the visualisation framework to implement the actual animation and transition. It is also dependent on the grammar and syntax of the visualisations themselves. Therefore, translating Deimos to other visualisation toolkits requires adaptation to support the new declarative grammar, and the toolkit itself needs to support animation between keyframes via interpolation. While it is technically possible to create a middleware to translate visualisation specifications and thus increase modularity, we did not explore this option in this work.


\subsection{XR Interactions}
We use the Mixed Reality Toolkit (MRTK)~\cite{microsoftMRTK} to enable XR interactions in Deimos. As a result, Deimos is able to be deployed on a range of platforms including Windows Mixed Reality, Oculus Quest, and HoloLens. However, due to the aforementioned performance limitations when working with large amounts of data, it is recommended to only use Deimos in tethered VR or remote MR setups. Both controller and articulated hand tracking are supported in Deimos in the form of source-based signals (see Section~\ref{sss: source-based-signals}). While Deimos does not support eye gaze or voice input, these can be included in future work.


% \subsection{Observable Streams and Signals} \label{ssc: prototype-signals}
% Signals in Deimos draw upon E-FRP principles~\cite{wanEventDrivenFRP2002}. Internally, Deimos constructs signals in the form of observable streams using the UniRx package~\cite{neueccUniRx}. For observables that can be easily shared across all visualisations in the scene (i.e., non-deictic signals, see Section~\ref{sss: source-based-signals}), they are instantiated once upon initialisation and re-used across multiple morphing visualisations. For non-shareable observables (i.e., deictic signals), they are created and destroyed at runtime as visualisations enter and exit the different states in the different morphs. These observables are combined and subscribed to where necessary, with all subscriptions being disposed of when a morph and its transitions are no longer valid.
% All expressions in Deimos, including those in signals and states, are evaluated using the DynamicExpresso package~\cite{dynamicExpresso}. We configured DynamicExpresso to support several custom functions (see Section~\ref{sss: expression-signals}). While more can be added by the user, this needs to be done in C\# at compile time.

==> original-sections/6._example-gallery.tex <==
\section{Example Gallery} \label{sec: example-gallery}
We present several examples of morphs created with the Deimos grammar. We categorise and describe the examples in three ways, with the first two aligning with the design goals in Section~\ref{sec: design-goals}.
First, we highlight how morphs can be designed to adapt to different visualisation configurations using generic states (DG1), but also allow for bespoke morphs by using specific states in controlled contexts (DG3).
Second, we demonstrate how morphs can be controlled using both embodied (DG2) and non-embodied (DG3) interaction methods. 
And third, we provide two scenarios in which Deimos can facilitate prototyping of different interaction methods in order to help evaluate the design of the grammar itself.
All examples and their specifications can be found in the Unity project files\footnote{Github link provided on acceptance. For review, the project files are instead provided in supplementary material.}. As such, we do not provide nor go into detail about each example's specification. The project files also contain additional example morphs not described in this paper.

%We present several examples of morphs created using the Deimos grammar. To demonstrate how the grammar achieves the design goals in Section~\ref{sec: design-goals}, we describe the examples in two different contexts: (i) the spectrum of dynamic morphs between generic and specific (DG1 and DG3); and (ii) the spectrum of interactions to enable morphs that range between embodied and non-embodied (WIMP-based) (DG2 and DG3). We also describe a third context which helps evaluate the design of the grammar itself: the interchangeability of signals to support rapid prototyping of different morph interactions.
%All examples and their specifications can be found in the Unity project files\footnote{Github link provided on acceptance. For review, the project files are instead provided in supplementary material.}. As such, we do not provide nor go into detail about each example's specification. The project files also contain additional example morphs not described in this paper. %Images of these examples are shown in Figures~\ref{fig:teaser}, \ref{fig:deimos-json}, and \ref{fig:deimos-example-gallery}, with intermediary stages and/or JSON shown for select morphs.


\subsection{Generic vs specific morph examples}
In DG1 and DG3, we described a spectrum in which morphs can vary between generic, adapting itself to a range of visualisation configurations, and specific, allowing it to be used in controlled settings.

On the generic end, we present the \textit{3D Barchart Partitioning and Stacking} morph (shown in Figure~\ref{fig:teaser}). It takes a 3D barchart and either partitions it into a 2D faceted barchart, or stacks it into a 2D stacked barchart whenever it touches a surface in the immersive environment. During the transition, it also aligns the visualisation to be parallel against the surface that it had touched. This is an example of a morph involving three states and two transitions in a branch-like structure. The triggers are set up so that the applied transition is based on the angle of contact between the barchart and surface: orthogonal for the faceted barchart, and parallel for the stacked barchart.
Its states are defined such that they only check that the encodings' types are correct (i.e., nominal \textit{x} and/or \textit{z}, quantitative \textit{y}) and that it uses cube marks. Through this, so long as a visualisation is a 3D barchart then it can undergo this morph, greatly expanding the range of scenarios which it can be used in. JSON path accessors are also used substitute in the proper field names during runtime (i.e., \textit{facetwrap}, \textit{yoffset}).

On the other end of the spectrum, the \textit{Geographic Scatterplot with Slider} morph (shown in Figure~\ref{fig:deimos-examples-slider}) demonstrates the use of two predefined states: a scatterplot and a choropleth map. Both of these are explicitly defined using exact encodings and field names (e.g., ``Population'', ``LifeExpectancy''). Because of this, only a visualisation with these exact encodings and fields can undergo this morph. A transition connects the two states together, which is controlled using a linear slider represented by a Unity GameObject. A signal accesses the \textit{x} position of this GameObject and uses it as the timing property of the transition.
A morph like this is useful for controlled settings like data-driven storytelling, as the visualisation(s) are all predefined by the author. %However of course, a DXR visualisation that directly corresponds with either state needs to also be created to see the effects of the morph.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{images/deimos-examples-slider.pdf}
    \caption{Still images of the \textit{Geographic Scatterplot with Slider} morph, using Unity GameObjects as a slider to control the transition.}
    \Description{A set of still images showing a hand moving a slider from left to right, which causes the points on a 2D scatterplot to move, and then expand into a choropleth map.}
    \label{fig:deimos-examples-slider}
\end{figure}

\subsection{Embodied vs non-embodied morph examples}
In DG1 and DG3, we described a spectrum in which morphs vary been the use of embodied vs non-embodied (or WIMP-based) interactions.

On the embodied end, the \textit{Barchart Unstacking} morph uses a ``pinch and pull'' gesture to unstack the bars of a 2D barchart into a side-by-side 3D barchart (shown in Figure~\ref{fig:deimos-examples-embodied} left). To strengthen the metaphor of bars being extruded out into 3D, a condition is added whereby the 2D barchart needs to be positioned against a surface for the morph to be allowed.
To initiate the transition, the user also needs to perform a pinch gesture on the visualisation itself, which is represented by a deictic signal. Other signals calculate the distance between the user's hand and the surface the visualisation is resting against.
The transition uses this distance as its timing property, causing the bars to extrude at the same rate which the user pulls away from them. In this fashion, the user perceives themselves as actually stretching the barchart into 3D. Of course, this is but one way in which embodied interaction can be achieved, but this approach can be replicated across other morphs to achieve similar styles of extrusion effects.

On the non-embodied end, the \textit{Menu-based Extrusion} morph adds a third spatial dimension to a 2D scatterplot, but does so via an MRTK toggle button~\cite{microsoftMRTK} (shown in Figure~\ref{fig:deimos-examples-embodied} right). A signal retrieves the state of this toggle button, and will trigger the visualisation when the button is toggled on. This example also demonstrates the use of a radial menu to select the field name of the newly added dimension. A signal retrieves the selected value and substitutes it into the 3D scatterplot state at keyframe creation.
In comparison to the \textit{Barchart Unstacking} morph, this example presents a much simpler and more familiar type of animated transition, albeit in an immersive environment.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{images/deimos-examples-embodied.pdf}
    \caption{Examples of embodied and non-embodied morphs. Left: Still images of the \textit{Barchart Unstacking} morph, using a ``pinch and pull'' gesture to unstack a 2D barchart into 3D. Right: The result of the \textit{Menu-based Extrusion} morph showing the radial menu and toggle button.}
    \Description{A two-part image. The first part shows a 2D barchart on a surface. A hand grabs onto this barchart and pulls away from it, causing the 2D barchart to extrude out into 3D, and level itself out into a 3D side-by-side barchart. The second part shows a 3D scatterplot. Next to it is a radial menu with the options ``Cylinders'', ``Displacement'', and ``Horsepower'', with Displacement being selected. Below it is a toggle button that is enabled labelled ``Extrude Visualisation''. The 3D scatterplot has a z dimension with the field Displacement.}
    \label{fig:deimos-examples-embodied}
\end{figure}


\subsection{Prototyping morph interactions} \label{ssc: example-gallery-prototyping}
Lastly, we demonstrate how the grammar allows for signals to be easily swapped and modified to allow rapid prototyping of different interactions. In terms of the Cognitive Dimensions of Notations~\cite{greenCognitiveDimensionsNotations1989}, this corresponds to a low level of \textit{viscosity}.

In this example, we recreate \textit{Tilt Map} by Yang et al.~\cite{yangTiltMapInteractive2020} using Deimos (shown in Figure~\ref{fig:deimos-examples-tiltmap} top).  Three states are defined: choropleth map, prism map, and barchart. Two transitions are defined to connect these states in a linear fashion. A signal is then created to retrieve the tilt angle of the visualisation relative to the horizontal plane. This tilt angle then subdivided into two ranges at specific angles using expression signals, that are then used as tweening variables for the two transitions (choropleth to prism, prism to barchart). With this setup, a visualisation will morph between the different states depending on its tilt.
However, we can easily change the manner which the morph is controlled just by replacing the tilt angle with some other source. A straightforward example is to replace it with the height of the visualisation relative to the floor (shown in Figure~\ref{fig:deimos-examples-tiltmap} bottom). The two expression signals which subdivide the range will also need to be updated to the new value ranges. In doing so we turn \textit{Tilt Map} into a so-called ``Height Map'', just by changing a few lines in the morph specification. The result is shown in Figure~\ref{fig:deimos-examples-tiltmap}.

\begin{figure*}[htb]
    \centering
    \includegraphics[width=\linewidth]{images/deimos-examples-tiltmap.pdf}
    \caption{Top: Still images of the \textit{Tilt Map} morph based on Yang et al.~\cite{yangTiltMapInteractive2020}. A red and green angle bracket is shown to provide rotation cues. Bottom: A modified version of \textit{Tilt Map} showing changes to the signal specification and the resulting morph shown as still images. This example shows tilt being replaced with height. A red and green bar is shown to provide height cues. }
    \Description{A two part image. The first part shows a series of still images of a 2D choropleth map being tilted. As it rotates, it morphs into a prism map. As it rotates even further, it morphs into a 2D barchart. The second part shows a modified version of the first part. Two signal specifications written in JSON are shown which shows the modifications made. Next to it are still images of a choropleth map turning into a prism map, then into a 2D barchart as it is lowered towards the ground.}
    \label{fig:deimos-examples-tiltmap}
\end{figure*}

Inspired by work on small multiple layouts in immersive environments~\cite{liuDesignEvaluationInteractive2020}, we created the \textit{Proxemic-based Facet Curvature} morph (shown in Figure~\ref{fig:deimos-examples-faceted} top). It morphs a faceted chart between three different layouts: flat, curved, and spherical. These three layouts correspond to three states in the morph, with two transitions connecting them linearly. A signal retrieves the distance between the user's head and the visualisation, with two more signals subdividing the distance into tweening variables (similar to the \textit{Tilt Map} morph). As the user approaches the faceted chart, it begins to wrap around them into a curved layout, and when they are close enough it morphs into an egocentric spherical layout.
To demonstrate another method of controlling this morph, we can replace the distance signal with the value of a rotary dial (shown in Figure~\ref{fig:deimos-examples-faceted} bottom). As the user rotates the dial the small multiples curve inwards or outwards. To do so, we create a separate cylinder GameObject in Unity which functions as this dial. We then replace the distance signal with a signal which retrieves the rotation value of the cylinder, and we also update the ranges of the two subdividing signals. This functionally turns the proxemics-based interaction into one involving the manipulation of an external object. This object is currently only virtual, but the concept can be applied to physical objects using either tangible input or motion tracking.
%Given their similarities, we can technically replace the signals in this morph from the ones in \textit{Tilt Map}. Instead, we will create a new cylinder GameObject in Unity which will act as a rotary dial. By replacing the distance signal with one that retrieves the rotation of this cylinder, we essentially turn the proxemics-based interaction into one involving the manipulation of an external object. While this object is still a virtual GameObject, this can easily be replaced with a physical object through either tangible input or motion tracking.

\begin{figure*}[htb]
    \centering
    \includegraphics[width=0.8\linewidth]{images/deimos-examples-facet.pdf}
5    \caption{Top: Still images of the \textit{Proxemic-based Facet Curvature} morph, which curves around the user based on distance between them and the chart. Bottom: A modified version which replaces distance with the rotation of a separate dial object. The changes to the signal specification are shown with the resulting morph shown as still images.}
    \Description{A two part image. The first part shows a series of still images of a faceted chart turning from a flat layout to a curved layout, then into a spherical layout, as a VR avatar approaches it. The second part shows a modified version of the first part. Two signal specifications written in JSON are shown which shows the modifications made. Next to it are still images of the same faceted chart going from flat to curved to spherical, but this time it is controlled using a virtual dial object.}
    \label{fig:deimos-examples-faceted}
\end{figure*}

==> original-sections/7._user-study.tex <==
\section{Expert Evaluation} \label{sec: user-study}
We conducted an evaluation of Deimos in order to: 
(i) determine the ease of use and expressiveness of the grammar; 
(ii) get impressions on the concepts introduced in the grammar; and 
(iii) generate discussion topics and research directions of the use of animated transitions in immersive environments.

\subsection{Study Design}
We use an approach similar to Zong and Pollock et al.~\cite{zongAnimatedVegaLite2022} by recruiting three developers of immersive analytics grammars and toolkits: Peter Butcher of VRIA~\cite{butcherVRIAWebBasedFramework2021}, Philipp Fleck of RagRug~\cite{fleckRagRugToolkitSituated2022}, and Ronell Sicat of DXR~\cite{sicatDXRToolkitBuilding2019}. 
To diversify our participant pool, we also recruited Zeinab Ghaemi of immersive geovisualisation~\cite{ghaemiProxemicMapsImmersive2022a}, Tica Lin of embedded sports visualisation~\cite{linTheQuestOmnioculars2022}, and Jorge Wagner of the VirtualDesk exploration metaphor~\cite{wagnerfilhoVirtualDeskComfortableEfficient2018}.
We hoped to learn how Deimos could be positioned within each researcher's respective works.
To minimise learning requirements, we only invited researchers who have experience working with Unity.

The user study was conducted remotely in three sections, repeated for each participant.
First, we conducted a 30 minute introductory session where we explained the goals of the study, demonstrated the examples in Section~\ref{sec: example-gallery}, and went through high level concepts of the grammar.
Second, we tasked participants to use Deimos unsupervised for at least 2.5 hours. They were given walkthroughs and documentation\footnote{Walkthroughs and documentation are provided in supplementary material.} to learn the grammar, and were encouraged to create their own morphs with some suggestions given to them.
Third, we held a one-hour semi-structured interview based around the aforementioned evaluation goals. We asked participants to show us their created morphs, and asked questions relating to each participant's own field of research.
Throughout the study period, we modified the documentation based on participant feedback. While we made bug fixes to Deimos where necessary, we did not add or change any features. Each participant was offered a AU\$150 gift card as compensation for their time.

The interviews were recorded and transcribed. The first author independently performed thematic analysis on all six transcriptions, with two other authors doing the same on three transcriptions each. The three authors then discussed and synthesised the main themes together, which form the structure of this section and the following Discussion section.


\subsection{Usability feedback}
We compile participant feedback based on a selection of the most relevant Cognitive Dimensions of Notations~\cite{greenCognitiveDimensionsNotations1989}. Rather than using the dimensions as heuristics --- a common approach in related works (e.g.,~\cite{satyanarayanDeclarativeInteractionDesign2014, satyanarayanCriticalReflectionsVisualization2019}) --- we use them from a usability perspective to evaluate the Deimos grammar. However, we provide self-evaluation for certain dimensions where relevant.


%Initial Impressions and Cognitive Dimensions}
%We coded the participants feedback and mapped their results to 

\textbf{Error proneness (likelihood of making errors).}
All participants spent the required 2.5 hours using the toolkit, however four of the six spent 7--8 hours using it. The initial reasoning given by most participants was that enjoyed their time with Deimos and learning how it worked. On further inspection however it was clear that this was in part due to the steep learning curve of the grammar, with Fleck commenting ``I don't feel that three hours are enough.'' We identified several potential causes of this, largely due to grammar's \textit{error proneness}.
First, many participants (Fleck, Ghaemi, Lin, and Wagner) were unfamiliar with the DXR grammar, with even Sicat not having used DXR for three years. As a result, two grammars needed to be learnt, naturally increasing learning time. As the Deimos grammar is intrinsically linked to its visualisation grammar (see Section~\ref{ssc: prototype-data-visualisations}), it is apparent that the choice of visualisation package brings not only technical but also notational difficulties.
Second, our documentation assumed full knowledge of Unity and its functions which not all participants had.
Third, the error messages provided by the Deimos prototype were not useful for participants. While the JSON schema validates whether the morph specification is syntactically correct before it is parsed, no check exists for semantic correctness (e.g., making sure \textit{name} properties are unique). This has since been corrected in the prototype.
Some participants suggested ways of easing the learning curve. Sicat suggested video tutorials to better explain the grammar, whereas Butcher suggested providing the DXR documentation as pre-reading before the study is even conducted. Interestingly, no participant suggested changes to the grammar itself beyond simple name changes (the terms \textit{signals} and \textit{restrict}). Whether this is due to participants not having had enough time to be exposed to Deimos' advanced features is unclear.

\textbf{Closeness of mapping (closeness to problem domain).}
The lack of grammar changes suggested by participants could be at least partially explained by its \textit{closeness of mapping}. All participants, when asked, had little to no issues understanding how the grammar models the state machine (see Figure~\ref{fig:deimos-state-machine-1}). The only participant who raised potential challenges was Fleck, citing the differences between declarative and imperative languages. As Unity primarily uses imperative programming, the shift to a declarative style in Deimos could cause confusion to certain users, particularly when constructing an interaction using signals. We don't believe this to be a major issue however, especially if the immersive visualisations also use a declarative language (e.g., DXR~\cite{sicatDXRToolkitBuilding2019}, VRIA~\cite{butcherVRIAWebBasedFramework2021}).

\textbf{Viscosity (resistance to change).}
After following the walkthroughs, all participants used the same strategy of combining parts of existing examples together to create new morphs to facilitate their learning. For example, Wagner combined the states and transitions of \textit{Tilt Map} example and the signals of the \textit{Proxemic-based Small Multiple Curvature} example to create a rudimentary ``Proxemic Map''. There are only a few examples of participants extending existing examples with completely new components: Sicat remapped the proxemic interaction of the \textit{Proxemic-based Small Multiple Curvature} example with a virtual rotary dial (the same as in Section~\ref{ssc: example-gallery-prototyping}), and Butcher created a stacked barchart to side-by-side barchart morph based on whenever the mouse is clicked. These all demonstrate a low level of \textit{viscosity} within the grammar, as participants were generally able to achieve their goals without issue (minus the aforementioned issues regarding error proneness). The same concept was also described in Section~\ref{ssc: example-gallery-prototyping}.
However, poor error messages introduced viscosity for a few participants. For instance, Lin had tried to create a reduced version of the \textit{3D Barchart Partitioning} example by removing all surface related signals, but the toolkit did not warn her to remove the references to these signals in the states, resulting in errors. This need to keep track of changes in multiple parts of the specification contributes to higher viscosity.

% \textbf{Visibility (ability to view components easily) \& Consistency (guessability of notation).}
\textbf{Visibility (ability to view components easily).}
Several participants (Fleck, Sicat, and Ghaemi) noted issues relating to the \textit{visibility} of signals in the grammar, primarily due to the large number of possible keywords involved. It was not obvious what options and/or combinations of signals are available without resorting to the documentation, although the JSON schema aided this process. The same participants acknowledged however that this reliance on documentation is fairly normal for toolkits, especially with only a few hours of experience.
From a technical perspective, the Deimos prototype improves visibility by exposing the names of any active morphs and/or transitions on each visualisation, and provides a toggle to print the emitted values of signals to the console for debug purposes. Further debug messages can also be enabled which shows the visualisation specifications of generated keyframes in JSON format. While these features were not explained in the documentation, they were highly useful during the development of Deimos and the creation of our example gallery.
%they were highly useful when helping participants debug their morphs during the interview.
%Lastly, Sicat had mentioned that he tried to skip ahead of the walkthrough and start creating his own morphs, but quickly became stuck on the more advanced functionalities, indicating a low level of \textit{consistency}.

==> original-sections/8._discussion.tex <==
\section{Discussion} \label{sec: discussion}
This section continues from Section~\ref{sec: user-study} by summarising the main themes and discussion topics of the semi-structured interviews with our expert participants.

\textbf{Adaptive morphs.}
While some participants liked the concept of adaptive morphs, others found it getting in the way of their authoring process.
Butcher saw value in adaptive morphs, saying ``I could see why that would be useful, especially if you had a large array of different charts... having it modular just makes sense.''
Wagner thought that ``the premise works well'', but clarified that he would prefer to have ``a [morph] specification for each type of graph'' instead of one hyper-generic morph that applies to all visualisation idioms.
Ghaemi was caught off-guard by this function when her new morph was being applied to other visualisations unintentionally (a result of overly generic states), but was able to reason with modifying the states to ensure that they are more specific.
Fleck and Sicat faced a similar issue, but instead suggested the ability to use an ID to directly target a specific visualisation, skipping the state matching process altogether. This was particularly of relevance to Fleck, where in \textit{RagRug}~\cite{fleckRagRugToolkitSituated2022} ``the user does not create a visualisation [themselves], but the system creates the existing visualisations.''
Overall, participants were able to grasp the concept of adaptive morphs, but it is apparent that their experiences come from the perspective of the morph author. A quantitative evaluation involving data analysis utilising pre-made morphs for practical tasks would be needed to fully evaluate the concept.

% Participants had varied opinions on the usefulness of adaptive morphs (DG1).
% For Fleck and Sicat, it got in the way of creating new morphs as it would inadvertently affect other visualisations in the environment, particularly if the states were not yet configured correctly. Both suggested the ability to match states based on the name or ID of a specific visualisation. This was particularly of relevance to Fleck, where in \textit{RagRug}~\cite{fleckRagRugToolkitSituated2022} ``the user does not create a visualisation [themselves], but the system creates the existing visualisations.''
% Butcher had a positive outlook on this, saying ``I could see why that would be useful, especially if you had a large array of different charts... having it modular just makes sense.'' This statement however was made in the context of applying the same morph to multiple views at once, instead of a single visualisation being able to undergo multiple morphs throughout its lifespan.
% Lastly, Wagner found the grammar easy to use when working with very specific rules and fields, but had some difficulties making them more generic, particularly due to his inexperience with DXR. He said it would be more likely that he ``would have some rules for scatterplots, and then histograms and things like that'', which is similar in specificity to many of our examples in Section~\ref{ssc: example-gallery-embodied-morphs}.
% While opinions did vary, ultimately our participants were authoring morphs in a very controlled setting. A quantitative evaluation involving end-users utilising morphs for practical tasks would be needed to fully evaluate the concept.

\textbf{The purpose of morphs.}
All participants found the examples exciting and interesting, but some had thoughts on their actual purpose. Ghaemi said that morphs are mainly useful when they add or change the data shown, rather than simply remapping encodings (e.g., \textit{Stacked Barchart Extrusion} example).
Lin similarly said that she would only use morphs when working with large amounts of data, such as combining proxemics with Shneiderman's mantra~\cite{shneidermanEyesHaveIt1996}, or when working with multiple views, but ``if it's only one smaller data set, and one chart, I probably wouldn't use it to morph between different columns.''
Butcher said that while our example morphs were ``neat and novel'', their animations did not strictly reveal new information, such as a time varying scatterplot does. %He argued for proper use cases and application scenarios to better demonstrate the usefulness of morphs.
Therefore, future work should investigate specific use cases for morphs and how morphs may potentially vary between them. 
%Therefore, while we still believe that Deimos shows promise in creating a range of interesting and compelling morphs, further investigation of different use cases and domains is need to properly assess and extract their value.


\textbf{Embodied interaction and discoverability.}
The reception to the use of embodied interactions in Deimos (DG2) was positive, but two participants raised discussion topics around their long term effects. Many of our example morphs use interaction metaphors for embodied interaction (e.g., collide with surface, pinch and pull). Sicat expressed concern over the use of these metaphors, saying ``...maybe in my application, pinning to the wall means or does something, and then someone else develops a morph where stick to the wall does something else... that might confuse people... there's no universal rule that says, pinning to the wall should do this.'' When asked if Deimos could play a role in shaping these metaphors, Sicat responded ``I would keep it open for now and just let [researchers] explore'', noting that the field is still not mature yet. He then suggested the use of tooltips to guide users in discovering morphs, especially when conflicting metaphors are used, but stated this is of low priority. In a similar vein, Lin suggested two ways of improving embodied morphs and their discoverability, especially as she had difficulties performing the rotation required for the \textit{3D Barchart Partitioning and Stacking} example. The first was to have the system predict what action the user is about to do, and display the morphs associated with that action in a ``gestural menu'' that the user can select to trigger the morph. The second was to show a preview of the morph while performing the interaction. When asked about the importance of these features, she said that they ``probably [don't] affect the current grammar, because it's more like an assistant towards the completion of certain interactions'', and that they are more like external scripts loaded after the core grammar. Overall, while there are broader implications of the use of embodied interaction in immersive analytics, we see power in Deimos being used to explore this design space in the long term, rather than immediately prescribing them in this work.


\textbf{GUIs and morph templates.}
Fleck, Sicat, and Ghaemi brought up ideas on how GUIs can be incorporated into Deimos. Fleck suggested the use of data flows in Node-RED to author morph specifications in JSON, similar to how visualisation specifications are created in \textit{RagRug}~\cite{fleckRagRugToolkitSituated2022}. Sicat recalled his own experiences developing DXR's GUI~\cite{sicatDXRToolkitBuilding2019}, noting that a GUI can be useful for non-experts and even end-users to create their own morphs. In a similar vein, Ghaemi said that a GUI would have greatly assisted her learning process with Deimos, citing her lack of experience in both DXR and toolkits in general. However, both participants clarified that the GUI should only cover basic functions, and advanced features should only be accessed in JSON format. 
Sicat went on to suggest that the GUI could expose templates for different parts of the grammar that allows users to mix and match and create new morphs with, which would be exposed through dropdowns and menus. He compared this idea to how he used the grammar himself, saying ``I went through your examples, copied the morphs and then pasted it into my morphs and then just modified them a bit. So it's kind of same idea, right? Just a different interface. So for non experts [it] would be super easy.''
Lin suggested something similar except from an interaction perspective, especially as in our included examples ``the interaction you perform is very standardised.'' This feedback opens many future design possibilities for how a GUI for toolkits like Deimos might look like, especially if it can allow end-users in VR or MR to create and/or modify their own morphs to suit their own needs without needing to write JSON.

\textbf{Inspiration drawn from the toolkit.}
All participants drew interesting comparisons between Deimos and their respective works. Wagner, Ghaemi, and Lin all showed great interest in morphs that transition between 2D and 3D. For Wagner, from the context of his work on VirtualDesk~\cite{wagnerfilhoVirtualDeskComfortableEfficient2018}, said ``it would be very interesting to be able to just snap [3D visualisations] to the desk, and then they project to 2D, which is something that many experts are very comfortable with, but then I could show to them that they can extract [the visualisation] from the desk or from the wall, and try to grab it and look around...'' For Ghaemi whose field is immersive geovisualisation~\cite{ghaemiProxemicMapsImmersive2022a}, it was to have the morph directly tied to adding layers to a virtual map, ``[when the] 3D chart collides with the map, the bars could be scattered through the buildings, so I can see the charts on top of the building.'' For Lin, she raised ideas in the context of embedded sports visualisation~\cite{linTheQuestOmnioculars2022}, whereby ``you [can] drag the 2D charts onto a specific player, or maybe drag it onto the court, like the flat ground floor, and then it just suddenly morphs into this heatmap.'' In this sense, rather than a visualisation just morphing between 2D and 3D, it could also morph between being embedded and non-embedded~\cite{willettEmbeddedDataRepresentations2017}.
We then asked whether they could see themselves using Deimos to aid in their research.
Wagner thought that as a proof of concept it would work ``super well'', but cited poor scalability of the toolkit as a reason against using it.
%Wagner cited Deimos' poor performance as the main reason against using it, which is mainly the result of DXR's infrastructure.
Ghaemi was receptive, hypothesising that ``the [toolkit] that you have it's, at least, for some of [my ideas], I'm pretty sure that I can implement what I want''. She also noted that there are no other immersive analytics toolkits that currently enable animated transitions in the manner she desired. Lin said that ``there's a high chance that I could use this library to help me prototype some scene to show [sports analysts and coaches]''. After this proof of concept stage however, she would instead develop her own research prototype from the ground up to support specific features such as ``instant data updating''.
Lastly, Butcher said that ``seeing the change in data and understanding what you know, getting something out of it, it's important... certainly not enough attention has been paid to it in the past I don't think, especially in the immersive space.'' He followed this up by saying ``it's definitely something we're going to look at in future for sure, the effect is fantastic.''
While it is expected that not every researcher can make use of the Deimos grammar and the toolkit, our user study clearly demonstrates the significance of this work in generating further research ideas and promoting the study of animated transitions in immersive analytics.

\section{Limitations}
Our work naturally has several limitations in regards to the grammar, the technical implementation, and the user study. First, our grammar is built upon several key concepts such as dynamic morphs and embodied interaction. While we aimed to justify these ideas in Section~\ref{sec: design-goals}, we did not properly evaluate them with actual end-users in VR/MR performing data analysis tasks. Therefore, we cannot confidently say that our approach is quantifiably beneficial for immersive analytics.
Second, our participants were not exposed to all of the functionalities of Deimos. It is certainly possible that there are pain points when using Deimos' advanced functionalities which were not identified due to the limited amount of time participants spent using it. This could include the inability to perform certain embodied gestures with the grammar, or difficulties managing morphs that contain more than 2 or 3 states and/or transitions.
Third, as the grammar is dependent on the visualisation package that it is built upon, many of its limitations are born from DXR~\cite{sicatDXRToolkitBuilding2019}. Limitations include the inability to transition between different mark types, lack of runtime data transformations, and overall poor scalability compared to other toolkits like IATK~\cite{cordeilIATKImmersiveAnalytics2019} especially when rendering large amounts of data. The inability to transform data (e.g., aggregation and filtering) is especially troublesome as it meant that time varying animations (e.g., Gapminder~\cite{roslingGapminder2007}) were not considered while designing the grammar, and using certain visualisations in morphs such as barcharts required pre-processing. While we had attempted to add data transformations into DXR ourselves, the challenges in using .NET as a scripting language made it difficult to achieve a syntax remotely equivalent to that of Vega-Lite~\cite{satyanarayanVegaLiteGrammarInteractive2017}. We see this as obvious future work, especially as it can allow visualisations to morph not just between encodings, but also between different levels of aggregation, filters, or even different datasets.

==> original-sections/9._conclusion.tex <==
\section{Conclusion} \label{sec: conclusion}
This paper presented Deimos, a grammar and toolkit for prototyping morphs in immersive environments. Morphs are a collection of animated transitions that occur between different defined states, which are triggered and modified by the use of signals. These morphs are dynamically applied to visualisations during runtime, and are designed to leverage embodied interaction to enable interactive animated transitions. We view Deimos as an initial foray into what a functional grammar to create embodied animated transitions in immersive environments would look like. While our example gallery and user study demonstrates Deimos' ability to create a wide range of morphs, future work would seek to understand how these morphs are used by actual data analysts and/or audiences of immersive data stories in VR/MR. We also hope that this work fuels greater interest in the use of dynamically morphing visualisations in immersive analytics.
